MP2: A Momentum Contrast Approach for Recommendation with Pointwise and Pairwise Learning

Binary pointwise labels (aka implicit feedback) are heavily leveraged by deep learning based recommendation algorithms nowadays. In this paper we discuss the limited expressiveness of these labels may fail to accommodate varying degrees of user preference, and thus lead to conflicts during model training, which we call annotation bias. To solve this issue, we find the soft-labeling property of pairwise labels could be utilized to alleviate the bias of pointwise labels. To this end, we propose a momentum contrast framework (MP2) that combines pointwise and pairwise learning for recommendation. MP2 has a three-tower network structure: one user network and two item networks. The two item networks are used for computing pointwise and pairwise loss respectively. To alleviate the influence of the annotation bias, we perform a momentum update to ensure a consistent item representation. Extensive experiments on real-world datasets demonstrate the superiority of our method against state-of-the-art recommendation algorithms.

==> pairwise_weight_pic.tex <==

\begin{figure}
%--1st pic--
\raggedright
\subcaptionbox{HR@5 \label{fig:subfig18}}{%
%\begin{subfigure}[b]{0.2 \textwidth}
\raggedright
\begin{tikzpicture}[scale=0.5]
\begin{axis}[
    xlabel={$\beta$},
    %ylabel={NDCG},
    xmin=1, xmax=8,
    ymin=0.15, ymax=0.7,
    xtick={1,2,3,4,5,6,7,8},
    xticklabels={0.0,0.1,0.5,0.9,0.99,0.999,0.9999,1},
    %ytick={0.3,0.4,0.5,0.6,0.7,0.8 },
    %legend pos=north west,
    legend style={ legend columns=2},
    ymajorgrids=true,
    grid style=dashed,
]

    \addplot[
    color=cyan,
    mark=asterisk,
    line width=2pt,
    ]
    coordinates {
    (1,0.5159936658749009)(2,0.4930720506730007)(3,0.5056215360253362)(4,0.5092636579572446)(5,0.5382422802850358)(6,0.5491290577988917)(7,0.4607917656373714)(8,0.4528899445764054)
    };
   \addlegendentry{Movielens-100k}
     
    \addplot[
    color=blue,
    mark=square,
     line width=1pt,
    ]
    coordinates {
  (1,0.327805135)(2,0.337976316)(3,0.336408137)(4,0.361871263)(5,0.373657521)(6,0.382495017)(7,0.3634482)(8,0.170491851)

    };
     \addlegendentry{Movielens-1M}
     
 \addplot[
    color=red,
    mark=*,
    line width=1pt,
    ]
    coordinates {
    (1,0.313250767)(2,0.277443532)(3,0.315985134)(4,0.307033582)(5,0.284087961)(6,0.31747277)(7,0.273723928)(8,0.263884942)
%(1,0.142107)(2,0.135222)(3,0.123485)(4,0.135712)(5,0.107213)(6,0.116995)(7,0.13854) #verison1
    };
    \addlegendentry{Beauty}
     
 \addplot[
    color=violet,
    mark=diamond,
    line width=2pt,
    ]
    coordinates {
    (1,0.246519102)(2,0.249420605)(3,0.240412819)(4,0.235411009)(5,0.251217635)(6,0.262683324)(7,0.258039109)(8,0.249782727)
    };
   \addlegendentry{Office Products}    
   
   
     
\end{axis}
\end{tikzpicture}
}
\subcaptionbox{NDCG@5 \label{fig:subfig2}}{%
%\end{subfigure}
%\hfil  \hfil  \hfil  
%\begin{subfigure}[b]{0.2  \textwidth}
\raggedleft
 \begin{tikzpicture}[scale=0.5]
\begin{axis}[
    xlabel={$\beta$},
    %ylabel={NDCG},
    xmin=1, xmax=8,
    ymin=0.1, ymax=0.6,
    xtick={1,2,3,4,5,6,7,8},
    xticklabels={0.0,0.1,0.5,0.9,0.99,0.999,0.9999,1},
    ytick={0.2,0.3,0.4,0.5,0.6,0.7,0.8 },
    %legend pos=outer north west,
    legend style={ legend columns=2},
    ymajorgrids=true,
    grid style=dashed,
]

    \addplot[
    color=cyan,
    mark=asterisk,
    line width=2pt,
    ]
    coordinates {
    (1,0.4405626911239629)(2,0.4201842319342088)(3,0.4242725017760578)(4,0.4379470710367412)(5,0.45951906836060125)(6,0.47399387638283397 )(7,0.3873084902818337)(8,0.37411131772280914)
    
    };
   \addlegendentry{Movielens-100K}
      
\addplot[
    color=blue,
    mark=square,
     line width=1pt,
    ]
    coordinates {
 (1,0.290748473)(2,0.294479451)(3,0.299099177)(4,0.32276111)(5,0.332032181)(6,0.3487884)(7,0.3368769)(8,0.143320765)

    };
     \addlegendentry{Movielens-1M}
     
 \addplot[
    color=red,
    mark=*,
    line width=1pt,
    ]
    coordinates {
     (1,0.165618626)(2,0.145123647)(3,0.166865602)(4,0.160383578)(5,0.145728174)(6,0.168056611)(7,0.139440674)(8,0.134243439) 
    };
    \addlegendentry{Beauty}
   
 \addplot[
    color=violet,
    mark=diamond,
    line width=2pt,
    ]
    coordinates {
     (1,0.133657521)(2,0.134884881)(3,0.127180272)(4,0.123253839)(5,0.135435851)(6,0.141565033)(7,0.136960116)(8,0.130082457)

    };
   \addlegendentry{Office Products} 
   
\end{axis}
\end{tikzpicture}    
%\end{subfigure}     
}

 \caption{ Performance of different pairwise loss weight $\beta$.}
\label{exp:pairwise_weight}
\end{figure}


==> preliminaries.tex <==
\section{Preliminaries}
\label{sec:model}
%In this section, we first introduce the problem setup and the preliminaries with regard to pointwise and pairwise learning. Then, we present the overall structure of our \method{} framework and explain its components in detail. At last we discuss the relation between \method{} and  prior models.

% \subsection{Problem Setup}
The most popular form of recommendation is to show an ordered list of items that will be of users' interest. The workflow of recommendation is first predicting preference scores of a candidate item set, and then delivering a small subset of candidates with top prediction scores. Recommendation algorithms mainly differ in how to predict item scores for users. Typically, pointwise methods utilize users' absolute preference (e.g., click or not click, purchase or not purchase) to learn models, and their data sample follows the format of $(U_i,V_j,y_{ij})$, where $U_i$ indicates the feature of user $i$,  $V_j$ indicates the feature of item $j$, and $y_{ij}$ is a binary label indicating user $i$'s absolute preference towards item $j$. In contrast, pairwise methods learn comparative preference and their training data format is is $(U_i,V_j,V_t, j>_{u}t)$, where $ j>_{u}t$ indicates whether user $i$ prefer item $j$ over item $t$.
 
In this paper, we combine the idea of pointwise and pairwise learning, and the training data format is $(U_i,V_j,V_t,y_{ij},y_{it},j>_{u}t)$. Specifically, one data sample contains three labels: two pointwise labels and one pairwise label. Next we describe three preliminaries that forms the basis of our framework.  

\begin{figure}[t]
\centering 
\includegraphics[width=.45\textwidth]{figs/preliminary.pdf}
%\includegraphics{SERecmodel1.pdf}
\caption{A graphical model of Two-tower structure and Embedding layer.}
\label{two_tower_mlp}
\end{figure}

%\subsection{Preliminaries}


\subsection{Learn to Rank (LTR)} Traditional LTR methods differ primarily in how they define surrogate loss functions over ranked lists of items during training, and they often are classified into three categories: pointwise, pairwise, and listwise (not in the scope of this paper) methods.  Pointwise methods approximate ranking to a classification problem and as such attempt to optimize the discrepancy between individual ground-truth labels and the absolute magnitude of relevance scores produced by the LTR model. There are numerous variants of pointwise and pairwise loss functions. We choose two differentiable losses that are widely used in practice. For pointwise loss, we choose the sigmoid cross-entropy for binary relevance labels $y_j \in \{0, 1\}$, which is computed as follows:

\begin{equation}
L_{pointwise} (\bm{y}, \hat{\bm{y}}) = - \displaystyle\sum_{j=1}^n  y_j \log(p_j) + (1-y_j) \log(1-p_j),
\label{eq:point_loss}
\end{equation}
where $p_j = \frac{1}{1 + \exp(-\hat{y}_j)}$, $\hat{y}_j$ is the predicted score, and $y_j$ is the truth label. As for pairwise loss, the pairwise logistic loss is defined as: 

\begin{equation}
L_{pairwise} (\bm{y}, \hat{\bm{y}}) = \displaystyle\sum_{u=1}^m \displaystyle\sum_{j=1}^n \displaystyle\sum_{t=1}^n  \mathbb{I}(y_j >_{u} y_t) \log(1 + \exp(-\hat{y}_{pair}))),
\label{eq:pair_loss}
\end{equation}
where $\mathbb{I}(\cdot)$ is the indicator function, $\hat{y}_{pair} = \hat{y}_j - \hat{y}_t$, and $\mathbb{I}(y_j >_{u} y_t) = 1$ indicates user $i$ prefer item $j$ over item $t$. Here $m$ and $n$ denote the number of users and items respectively.



\subsection{Embedding + MLP}
\label{embed+mlp} Compared with traditional recommendation algorithms, one advantage of deep learning-based models is their superiority in leveraging both numerical and categorical features. Numerical features are often rescaled due to skewed distributions or varying scales. Normalization and symmetric logarithm are two widely used feature transformation methods. For categorical features, embedding lookups are adopted to encode discrete values to vectors of real numbers. In particular, each embedding lookup may be interpreted as using a one-hot vector $\bm{e}_i$ (with the $i$-th position being $1$ while others are $0$, where index $i$ corresponds to $i$-th category) to obtain the corresponding row vector of the embedding table $W \in \mathbb{R}^{k \times d}$ as follows
\begin{equation}
\bm{w}_i^{T} = \bm{e}_i^{T} W.
\end{equation} 
In more complex scenarios, an embedding can also represent a weighted combination of multiple items, with a multi-hot vector of weights $\bm{a}^T = [0,...,a_{i_1},...,a_{i_k},...,0]$, with elements $a_{i} \ne 0$ for $i = i_1, ..., i_k$ and $0$ everywhere else, where $i_1, ..., i_k$ index the corresponding items. Note that a mini-batch of $t$ embedding lookups can hence be written as
\begin{equation}
    S = A^{T} W,
    \label{eq:batchedlookup} 
\end{equation}
where sparse matrix $A = [\bm{a}_1,...,\bm{a}_t]$. A graphical description of embedding is shown in Figure \ref{two_tower_mlp}.

Embeddings are often followed by multi-layer perceptron (MLP), the most fundamental component in deep learning. MLP consists of a prediction function composed of an interleaving sequence of fully connected (FC) layers and an activation function $\sigma : \mathbb{R} \rightarrow \mathbb{R}$ applied componentwise as shown below:
\begin{equation}
    \hat{y} = W_k \sigma( W_{k - 1} \sigma( ... \sigma( W_1 \bm{x} + \bm{b}_1 ) ...) + \bm{b}_{k - 1} ) + \bm{b}_k,
    \label{eq:mlp}
\end{equation}
where the weight matrix $W_l \in \mathbb{R}^{n_l \times n_{l - 1}}$, bias $\bm{b}_l \in \mathbb{R}^{n_l}$ for layer $l=1,...,k$. 
It has been shown MLPs with sufficient depth and width can fit data to arbitrary precision \citep{bishop1995neural}. Empirical results have shown that the combination of embedding + MLP could help to capture more complex interactions and thus improve recommendation performance. 



\subsection{Two-Tower Structure} 
This structure is widely applied by deep neural network models, which has two separate subnetworks that learn user representations and item representations separately. This design is originated from latent factor models (e.g., probabilistic matrix factorization~\citep{mnih2007probabilistic}), and a typical prediction in recommendation is computed by multiplication of a user representation and an item representation, namely $y_{ij}=u_iv_j$. One advantage of the two-tower structure in practice is that we can pre-store item representations in servers and only user representations are calculated in real time, which would save a lot of inference time since the size of candidate items is always very large. A graphical model of a two-tower structure is shown in Figure \ref{two_tower_mlp}.

==> relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}
\subsection{Deep Neural Networks in Recommendation}
 In recent years, deep neural networks (DNNs) have become successful in recommendations, some representative examples are PNN \citep{qu2016product}, Wide\&Deep \citep{cheng2016wide}, DeepFM \citep{guo2017deepfm}, and DLRM \citep{naumov2019deep}. To avoid manually building up high-order cross features, these methods attempt to automatically learn low-order and high-order interactions from numerical and categorical features. Empirical experiments have shown promising results of DNNs to learn sophisticated and selective feature interactions. However, these methods fall into pointwise learning, leaving pairwise and listwise learning (beyond the scope of this work) almost blank in deep recommendations. In traditional LTR studies \citep{burges2005learning,cao2007learning,rendle2014improving}, pairwise learning has shown superiority over pointwise learning so it is worth exploring deep models in pairwise learning scenarios. Few works have exploited pairwise learning for deep recommendation.  \citet{song2018neural} proposed a neural collaborative ranking model (NCR) that extends Bayesian neural ranking (BPR \citep{rendle2012bpr}) via learning user and item representations with two neural networks.

There also exists researches \citep{chen2015fusing,wang2016ppp,lei2017alternating,cinar2020adaptive} combining pointwise and pairwise learning, most of which focuses on designing a mixed loss function. For example, \citet{lei2017alternating} formulates an adaptive strategy as minimizing a particular objective function that generalizes the traditional pointwise and pairwise loss function. \citet{cinar2020adaptive} proposes a joint learning model (APPL) that alternately draw pairwise and pointwise data samples, optimizing the respective losses. Different from the previous studies, we take the model structure and loss functions (i.e., pointwise and pairwise losses) in a unified perspective.


 
%[46] proposes a Factorisation-machine supported Neural Network (FNN) to learn high-order feature interactions. It uses the pre-trained factorization machines for field embedding before applying DNN. [31] further proposes a Product-based Neural Network (PNN), which introduces a product layer between embedding layer and DNN layer, and does not rely on pre-trained FM. The major downside of FNN and PNN is that they focus more on high-order feature interactions while cap- ture little low-order interactions. The Wide\&Deep [5] and DeepFM [9] models overcome this problem by introducing hybrid architec- tures, which contain a shallow component and a deep component with the purpose of learning both memorization and generalization. Therefore they can jointly learn low-order and high-order feature interactions.

\subsection{Representation Learning with Momentum}
%\textcolor{red}{Describe main idea of momentum and its advantage. List some examples.}

Momentum-based methods are intensively employed in the recent study in deep representation learning, of which the majority approaches require a set of \textit{slowly-progressing} parameter counterparts, updated with a momentum as reference during training. This idea has been proven to be fully functioning and effective in the context of self-supervised feature learning and pre-training in computer vision. Typical examples include momentum-based memory bank \cite{memorybank} and Momentum Contrast (MoCo) \cite{moco,mocov2}, with various extensions in other domains \cite{kang2020deep,xia2020self,chen2020momentum,lee2020momentum}. The community have also witnessed similar approaches with different terminologies such as temporal ensembling (the $\pi$ model) \cite{pimodel} and mean teacher \cite{mt} in semi-supervised learning, where either the exponential moving average or the momentum network literally shapes the \textit{slower} feature duplicates to be compared. 

However, we clarify that our proposed model differs from the aforementioned methods in motivation. Existing methods basically resort to the momentum-based approaches as a memory-saving solution to construct contrastive samples for comparison \cite{memorybank}, while we consider a slower evolving intensity with momentum on the item representations than the user ones throughout the training process for better performance. We also intentionally exclude the momentum-based SGD optimizers \cite{qian1999momentum,adam} from discussion as they ship different functionalities than this paper and are out-of-scope.

